Simulating Before Planning: Constructing Intrinsic User World Model for User-Tailored Dialogue Policy Planning

Recent advancements in dialogue policy planning have emphasized optimizing system agent policies to achieve predefined goals, focusing on strategy design, trajectory acquisition, and efficient training paradigms. However, these approaches often overlook the critical role of user characteristics, which are essential in real-world scenarios like conversational search and recommendation, where interactions must adapt to individual user traits such as personality, preferences, and goals. To address this gap, we first conduct a comprehensive study utilizing task-specific user personas to systematically assess dialogue policy planning under diverse user behaviors. By leveraging realistic user profiles for different tasks, our study reveals significant limitations in existing approaches, highlighting the need for user-tailored dialogue policy planning. Building on this foundation, we present the User-Tailored Dialogue Policy Planning (UDP) framework, which incorporates an Intrinsic User World Model to model user traits and feedback. UDP operates in three stages: (1) User Persona Portraying, using a diffusion model to dynamically infer user profiles; (2) User Feedback Anticipating, leveraging a Brownian Bridge-inspired anticipator to predict user reactions; and (3) User-Tailored Policy Planning, integrating these insights to optimize response strategies. To ensure robust performance, we further propose an active learning approach that prioritizes challenging user personas during training. Comprehensive experiments on benchmarks, including collaborative and non-collaborative settings, demonstrate the effectiveness of UDP in learning user-specific dialogue strategies. Results validate the protocol's utility and highlight UDP's robustness, adaptability, and potential to advance user-centric dialogue systems.

==> Tables/profile_compare.tex <==
\begin{table}[t]
    \caption{Generated profile example in P4G. The red part shows the correspondence between the profile and the task.}
    \vspace{-0.2cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c}
    \toprule
    \makecell[l]{\textbf{(\textcolor{blue}{Well-off}, \textcolor{blue}{Compassionate}, \textcolor{blue}{Rational})}: You are a 44-year-old \\
    urban farmer with a stable income that supports your sustainable \\
    agriculture endeavors. \textcolor{red}{Your compassionate nature drives you to} \\
    \textcolor{red}{support charitable causes that focus on food security and promot} \\
    \textcolor{red}{-ing healthy eating habits.} You believe in empowering communi\\
    -ties through access to fresh produce and nutritional education. \\
    \textcolor{red}{Your decision-making style is rational, as you carefully research} \\
    \textcolor{red}{and evaluate organizations that align with your values before} \\ 
    \textcolor{red}{making donations}.} \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{+0.1cm}
    \vspace{-0.3cm}
    \label{tab:illustration}
\end{table}
